Swift Linked Data Miner: Mining OWL 2 EL class expressions directly from online RDF datasets

In this study, we present Swift Linked Data Miner, an interruptible algorithm that can directly mine an online Linked Data source (e.g., a SPARQL endpoint) for OWL 2 EL class expressions to extend an ontology with new SubClassOf: axioms. The algorithm works by downloading only a small part of the Linked Data source at a time, building a smart index in the memory and swiftly iterating over the index to mine axioms. We propose a transformation function from mined axioms to RDF Data Shapes. We show, by means of a crowdsourcing experiment, that most of the axioms mined by Swift Linked Data Miner are correct and can be added to an ontology. We provide a ready to use Prot\'eg\'e plugin implementing the algorithm, to support ontology engineers in their daily modeling work.

==> stats-and-axioms.tex <==
\hline
& annotations:Comment \\
1 & terms:hasFormat \owlSome{} owl:Thing \\
2 & base:text \owlSome{} xsd:string \\
\hline
& annotations:Favourite \\
3 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& annotations:Rating \\
4 & annotations:rating-score \owlSome{} xsd:decimal[<= 5] \\
5 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& annotations:Tagging \\
6 & terms:hasFormat \owlSome{} owl:Thing \\
7 & annotations:uses-tag \owlSome{} owl:Thing \\
\hline
& annotations:Tag \\
8 & terms:title \owlSome{} xsd:string \\
9 & foaf:homepage \owlSome{} owl:Thing \\
10 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& credit:Attribution \\
11 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& credit:Creditation \\
12 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& base:ContentType \\
13 & terms:title \owlSome{} xsd:string \\
14 & terms:hasFormat \owlSome{} owl:Thing \\
15 & terms:type \owlSome{} xsd:string \\
16 & foaf:homepage \owlSome{} owl:Thing \\
\hline
& base:Friendship \\
17 & base:has-accepter \owlSome{} owl:Thing \\
18 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& base:Group \\
19 & ns:has_member \owlSome{} owl:Thing \\
20 & base:membership-policy \owlSome{} xsd:string \\
21 & ns:name \owlSome{} xsd:string \\
22 & foaf:homepage \owlSome{} owl:Thing \\
23 & terms:hasFormat \owlSome{} owl:Thing \\
\hline
& base:Membership \\
24 & terms:hasFormat \owlSome{} owl:Thing \\
25 & base:has-accepter \owlSome{} owl:Thing \\
26 & base:accepted-at \owlSome{} xsd:dateTime \\
\hline
& base:User \\
27 & terms:hasFormat \owlSome{} owl:Thing \\
28 & base:receive-notifications \owlSome{} xsd:string \\
29 & foaf:name \owlSome{} xsd:string \\
30 & ns:avatar value images:avatar.png \\
31 & ns:name \owlSome{} xsd:string \\
32 & foaf:homepage \owlSome{} owl:Thing \\
\hline
& components:BeanshellProcessor \\
33 & components:processor-type \owlSome{} xsd:string \\
34 & terms:title \owlSome{} xsd:string \\
35 & components:processor-type value "beanshell"^^xsd:string \\
\hline
& components:Content \\
36 & components:belongs-to-workflow \owlSome{} owl:Thing \\
37 & components:Content \\
\hline
& components:DataflowProcessor \\
38 & components:processor-type value "workflow"^^xsd:string \\
39 & terms:title \owlSome{} xsd:string \\
40 & components:processor-type \owlSome{} xsd:string \\
\hline
& components:Dataflow \\
41 & components:has-component \owlSome{} owl:Thing \\
\hline
& components:Input \\
\hline
& components:Link \\
\hline
& components:OtherProcessor \\
42 & terms:title \owlSome{} xsd:string \\
43 & components:processor-type \owlSome{} xsd:string \\
\hline
& components:Output \\
\hline
& components:Processor \\
44 & terms:title \owlSome{} xsd:string \\
\hline
& components:Sink \\
45 & terms:title \owlSome{} xsd:string \\
\hline
& components:Source \\
46 & terms:title \owlSome{} xsd:string \\
\hline
& components:Type \\
47 & components:Type \\
48 & components:belongs-to-workflow \owlSome{} owl:Thing \\
\hline
& components:WSDLProcessor \\
49 & components:service-name \owlSome{} xsd:string \\
50 & components:processor-type \owlSome{} xsd:string \\
51 & terms:title \owlSome{} xsd:string \\
\hline
& contributions:File \\
52 & base:has-policy \owlSome{} owl:Thing \\
53 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[>= "4"^^xsd:nonNegativeInteger] \\
54 & base:filename \owlSome{} xsd:string \\
55 & base:has-content-type \owlSome{} owl:Thing \\
56 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger \\
57 & base:has-current-version \owlSome{} owl:Thing \\
58 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[>= "1"^^xsd:nonNegativeInteger] \\
59 & ns:has_owner \owlSome{} owl:Thing \\
60 & terms:hasFormat \owlSome{} owl:Thing \\
61 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[<= "52604"^^xsd:nonNegativeInteger] \\
62 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[<= "7922"^^xsd:nonNegativeInteger] \\
63 & ns2:license value licenses: \\
64 & terms:title \owlSome{} xsd:string \\
65 & terms:created \owlSome{} xsd:dateTime \\
66 & base:content-url \owlSome{} owl:Thing \\
67 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger \\
68 & terms:modified \owlSome{} xsd:dateTime \\
\hline
& contributions:FileVersion \\
69 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[<= "7922"^^xsd:nonNegativeInteger] \\
70 & base:has-policy \owlSome{} owl:Thing \\
71 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[<= "52604"^^xsd:nonNegativeInteger] \\
72 & terms:title \owlSome{} xsd:string \\
73 & base:version-number \owlSome{} xsd:decimal[<= 7] \\
74 & terms:hasFormat \owlSome{} owl:Thing \\
75 & foaf:homepage \owlSome{} owl:Thing \\
76 & base:filename \owlSome{} xsd:string \\
77 & ns:license value licenses: \\
78 & base:version-number value 1 \\
79 & base:has-content-type \owlSome{} owl:Thing \\
80 & base:is-current-version value true \\
81 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger \\
82 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[>= "1"^^xsd:nonNegativeInteger] \\
83 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[>= "4"^^xsd:nonNegativeInteger] \\
84 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger \\
85 & base:content-url \owlSome{} owl:Thing \\
86 & base:is-current-version \owlSome{} xsd:string \\
\hline
& contributions:Workflow \\
87 & contributions:svg \owlSome{} owl:Thing \\
88 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[>= "4"^^xsd:nonNegativeInteger] \\
89 & contributions:thumbnail \owlSome{} owl:Thing \\
90 & terms:hasFormat \owlSome{} owl:Thing \\
91 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[>= "1"^^xsd:nonNegativeInteger] \\
92 & base:has-current-version \owlSome{} owl:Thing \\
93 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger \\
94 & base:has-content-type \owlSome{} owl:Thing \\
95 & contributions:thumbnail-big \owlSome{} owl:Thing \\
96 & contributions:preview \owlSome{} owl:Thing \\
97 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[<= "183188"^^xsd:nonNegativeInteger] \\
98 & ns:license \owlSome{} owl:Thing \\
99 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger \\
100 & base:has-policy \owlSome{} owl:Thing \\
101 & terms:title \owlSome{} xsd:string \\
102 & foaf:homepage \owlSome{} owl:Thing \\
103 & base:content-url \owlSome{} owl:Thing \\
104 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[<= "9683"^^xsd:nonNegativeInteger] \\
\hline
& contributions:WorkflowVersion \\
105 & base:version-number \owlSome{} xsd:decimal[<= 28] \\
106 & contributions:thumbnail-big \owlSome{} owl:Thing \\
107 & foaf:homepage \owlSome{} owl:Thing \\
108 & contributions:preview \owlSome{} owl:Thing \\
109 & terms:title \owlSome{} xsd:string \\
110 & base:is-current-version \owlSome{} xsd:string \\
111 & base:has-content-type \owlSome{} owl:Thing \\
112 & ns:license \owlSome{} owl:Thing \\
113 & terms:hasFormat \owlSome{} owl:Thing \\
114 & base:content-url \owlSome{} owl:Thing \\
115 & contributions:svg \owlSome{} owl:Thing \\
116 & base:has-policy \owlSome{} owl:Thing \\
117 & contributions:thumbnail \owlSome{} owl:Thing \\
\hline
& packs:LocalPackEntry \\
118 & terms:hasFormat \owlSome{} owl:Thing \\
119 & terms2:proxyFor \owlSome{} owl:Thing \\
\hline
& packs:Pack \\
120 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[<= "638"^^xsd:nonNegativeInteger] \\
121 & base:has-policy \owlSome{} owl:Thing \\
122 & foaf:homepage \owlSome{} owl:Thing \\
123 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger[>= "1"^^xsd:nonNegativeInteger] \\
124 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[<= "185582"^^xsd:nonNegativeInteger] \\
125 & terms:aggregates \owlSome{} owl:Thing \\
126 & terms2:title \owlSome{} xsd:string \\
127 & packs:has-entry \owlSome{} owl:Thing \\
128 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger[>= "6"^^xsd:nonNegativeInteger] \\
129 & viewings_downloads:downloaded \owlSome{} xsd:nonNegativeInteger \\
130 & terms:isDescribedBy \owlSome{} owl:Thing \\
131 & terms2:hasFormat \owlSome{} owl:Thing \\
132 & viewings_downloads:viewed \owlSome{} xsd:nonNegativeInteger \\
\hline
& packs:RemotePackEntry \\
133 & terms:proxyFor \owlSome{} owl:Thing \\
134 & terms2:title \owlSome{} xsd:string \\
135 & terms2:hasFormat \owlSome{} owl:Thing \\
\hline
& snarm:Policy \\
136 & terms:hasFormat \owlSome{} owl:Thing \\
137 & snarm:has-access value specific:PublicView \\
138 & snarm:has-access value specific:PublicDownload \\
\hline
& snarm:RestrictedAccess \\

